A Method for Multi-Robot Asynchronous Trajectory Execution in MoveIt2

This work presents an extension to the MoveIt2 planning library supporting asynchronous execution for multi-robot / multi-arm robotic setups. The proposed method introduces a unified way for the execution of both synchronous and asynchronous trajectories by implementing a simple scheduler and guarantees collision-free operation by continuous collision checking while the robots are moving.

==> chapters/experiments.tex <==

%The proposed system is expected to validate based on the ability to work, avoiding collisions. Also, the system is expected to validate against counterpart synchronous systems for time-varying tasks. The experiments will be carried out using two 7DoF PANDA robot arms in rviz software. 
